SPIRT: A Fault-Tolerant and Reliable Peer-to-Peer Serverless ML Training Architecture

The advent of serverless computing has ushered in notable advancements in distributed machine learning, particularly within parameter server-based architectures. Yet, the integration of serverless features within peer-to-peer (P2P) distributed networks remains largely uncharted. In this paper, we introduce SPIRT, a fault-tolerant, reliable, and secure serverless P2P ML training architecture. designed to bridge this existing gap. Capitalizing on the inherent robustness and reliability innate to P2P systems, SPIRT employs RedisAI for in-database operations, leading to an 82\% reduction in the time required for model updates and gradient averaging across a variety of models and batch sizes. This architecture showcases resilience against peer failures and adeptly manages the integration of new peers, thereby highlighting its fault-tolerant characteristics and scalability. Furthermore, SPIRT ensures secure communication between peers, enhancing the reliability of distributed machine learning tasks. Even in the face of Byzantine attacks, the system's robust aggregation algorithms maintain high levels of accuracy. These findings illuminate the promising potential of serverless architectures in P2P distributed machine learning, offering a significant stride towards the development of more efficient, scalable, and resilient applications.

==> 03.background.tex <==
\section{Background}
\label{sec:background}


\subsection{Serverless Computing for Training Distributed Machine Learning}



Serverless computing, an emerging paradigm in cloud computing, enables developers to build and deploy applications without managing server infrastructure. It removes concerns over infrastructure scaling and maintenance, freeing developers to focus on business logic. This paradigm has proven to be a powerful asset for distributed ML, providing scalable computational resources, cost-effectiveness, and effortless management of expansive applications. Nevertheless, the inherent statelessness of serverless computing requires the use of communication channels or databases to preserve transitional states, a key element in iterative ML model training.


\subsection{Redis and RedisAI}
Redis, an open-source, in-memory data structure store, serves as a database, cache, and message broker. The high-speed data access enabled by Redis's in-memory nature is particularly beneficial in serverless computing within distributed machine learning \cite{redis}.

RedisAI, an extension of Redis, integrates artificial intelligence capabilities into this high-performance database \cite{redisai}. As a model-serving powerhouse, RedisAI natively supports popular Deep Learning/Machine Learning frameworks and enables real-time AI operations, maximizing computational efficiency.

Importantly, the adaptability of RedisAI, given its support for multiple backends like TensorFlow, PyTorch, and ONNXRuntime, allows us to modify it for in-place model updates. This offers substantial efficiency improvements by eliminating the conventional read-process-write cycle in model updating.


\subsection{Robust aggregation in distributed ML}

Maintaining reliability in distributed learning systems hinges significantly on the adoption of robust aggregation strategies. These strategies play a critical role in the consolidation of local updates from various workers in the system. Traditional simple averaging methods for model updates are highly susceptible to outliers and discrepancies in data. The presence of such outliers can hinder system convergence or cause convergence towards a sub-optimal model.

Robust aggregation offers an effective countermeasure to these issues. By employing specialized processes to aggregate local updates, these strategies effectively manage outlier data, thereby enhancing the system's resilience and overall performance. In the following, we present the robust aggregation algorithms we utilized in this work.




\textbf{\textit{Medians-based robust aggregation \cite{xie2018generalized}:}} It is called as well robust aggregation rules, proven to be effective in combating Byzantine attacks. The Geometric Median (GeoMed) is a widely-used example of this. It constructs a vector that minimizes the overall distance to local updates from all workers, thereby lessening the influence of Byzantine workers. Another median-based approach is the Marginal Median (MarMed), which identifies the median value for each coordinate within the local updates. The resultant coordinate-wise medians form an output vector, creating a robust aggregation strategy.

\textbf{\textit{Zeno robust aggregation \cite{xie2019zeno}:}} It operates effectively as long as there's at least one healthy worker. ZENO uses a validation set to evaluate local updates, generating a score for each. Any update suspected of being malicious based on these scores is excluded, increasing the overall resilience of the aggregation process.



==> 06.Discussion.tex <==
\section{Discussions}
\label{sec:discussions}
--security and reliable ML:
secure communication etc, and robust aggregation.

While Marmed and Zeno take 8.2x and 5.9x more time than average aggregation, their ability to protect against Byzantine attacks and ensure model convergence validates this trade-off, highlighting their critical role in safeguarding ML operations.

--peer to peer based on serverless discussion... database reliablility, and how we solve it...

This phenomenon underscores a delicate balance that must be achieved in peer-to-peer decentralized networks for efficient model training. On one hand, we want to maximize parallelism, as this can potentially speed up model training. On the other hand, we must also manage the computational burden on each peer's database, as too many simultaneous computations (from a smaller batch size) or too heavy computations (from a larger batch size) can both lead to longer computation times.

% the total training time per epoch for both Densenet121 and MobileNet V3 Small models, respectively. We observe an overall decrease in training time per epoch with a larger batch size and a higher number of peers. Nonetheless, these tables also highlight the nonlinear relationship and the trade-offs between batch size and peers network scale. which open the door for future research to find the optimal architecture parameters for a specific model and dataset.

the fact that we are using a lambda to fetch gradients from other database is kind of used within Pytorch when it is activated in a distributed mode.


Logical peer to peer

how it is important to adapt the databases to make it follow the new waves using serverless computing to train machine learning in different architectur topologies.

lambda and heavy dependencies packages, open the doors for researchers to explore the way of tools that helps to reduce dependencies packages such as removing the documentations or pycache folders.


heartbeat discussion and the kind of architecture, you can implement heartbeat in many places inside the architecture accoriding to the system requirements to reduce the time that may takes to identify failed nodes.


discussion about the failure related to the channels we open with the database using sshtunnels is exhautive for database.

ReliabeleAI
the roles and accesses to different services is controlled as well by roles
\label{sec:discussion}

In this section, we delve into a thorough analysis of the experimental findings, scrutinizing their implications in relation to the overarching aim of our study: assessing the efficacy of the Serverless Peer Integrated for Reliable Training (SPIRT) architecture.

\subsection{Communication Overhead and Training Performance}

Our investigation into the relationship between communication overhead and training performance produced critical insights. Central to this relationship was the size of data batches processed concurrently. We observed a pronounced interdependence between batch size and both communication overhead with databases and training time.

Notably, the impact of batch size selection manifested consistently across various models and datasets, underscoring its universal importance in machine learning tasks. Too large a batch size might amplify communication overhead, while too small a size could potentially prolong the training time.

The intricate balance to be struck here brings to the fore the significance of carefully choosing an optimal batch size, ideally suited for the specific constraints of the serverless architecture and the particularities of the chosen models and datasets. As an extension of this finding, we posit that further research could be devoted to the development of dynamic batch size algorithms, designed to adaptively alter batch sizes according to the evolving dynamics of the training environment.

\subsection{Optimizing Communication Overhead with Redis}

Subsequent investigations compared the performance characteristics of model update operations and gradient averaging within the framework of standard Redis versus our bespoke RedisAI solution. The results attested to the remarkable potential of performing these computations directly within the database. This localized approach enabled us to bypass the typically repetitive fetch-update-store cycles, thereby significantly curtailing communication overhead and enhancing overall system efficiency.

These findings illuminate the benefits of incorporating in-database computations, especially within the realms of serverless distributed machine learning architectures. They also highlight an important research direction: exploring the extent to which computations can be embedded within databases to reduce communication overhead further and accelerate machine learning operations.

\subsection{Scalability and Fault Tolerance}

The robustness of SPIRT against alterations in network size - both due to the addition of new peers and the failure or removal of existing peers - was thoroughly assessed. In both scenarios, the architecture was capable of maintaining high performance levels while ensuring uninterrupted operation.

The architecture's response to peer failure was particularly implemented with AWS Lambda functions efficiently compensating for the computational capabilities of failed peers. However, an important aspect to note here is the duration between the detection of peer failures and the subsequent initiation of the new AWS Step Functions. Future iterations of the SPIRT architecture could focus on refining this aspect, aiming to minimize the delay and ensure an even smoother transition during peer failures.

Similarly, the addition of new peers to the network was managed proficiently, thereby demonstrating the inherent scalability of the architecture. However, a consequent rise in communication overhead was observed as the number of peers increased. This finding raises the need for advanced communication management strategies to sustain optimal performance as the network expands.

\subsection{Tolerating Byzantine Attacks}
\emna{i believe we can remove this pargraph}
The robustness of the SPIRT architecture was further evaluated under simulated Byzantine attacks. Our results unequivocally demonstrated the resilience of our architecture. The implemented robust aggregation mechanisms effectively detected and isolated the malicious behavior, thereby preserving the functional integrity of the network under adverse conditions. This showcases the importance of incorporating robust defensive strategies within serverless distributed machine learning architectures to safeguard against potential Byzantine attacks.


\subsection{Operational Consistency Across Diverse Models and Datasets}

In our study, we utilized a range of CNN models and datasets. An intriguing outcome of our analysis was the relative consistency in the architecture's operation across these different models and datasets. This consistency underlines the robustness of the architecture and its potential for generalization across various machine learning tasks.

Nevertheless, future investigations could aim to widen the array of models and datasets used. These might include more complex models and larger datasets to further test and improve the architecture's capabilities.

\subsection{Security Considerations}
\emna{not sure if you wanna keep this}
While our architecture demonstrated substantial resilience against Byzantine attacks, security within distributed machine learning environments remains a critical area for continual enhancement. As machine learning technologies become more advanced, so too do potential attack vectors.

Future work should prioritize the development and integration of advanced security measures to further fortify the network against potential attacks. These might involve leveraging advanced cryptographic techniques, refining the robust aggregation mechanisms, or incorporating additional mechanisms for anomaly detection and mitigation.

\subsection{Exploring Alternative Cloud Platforms}

Our architecture was primarily built on AWS services. However, the principles of serverless computing and distributed machine learning are applicable across various cloud platforms, including Google Cloud Platform (GCP) and Microsoft Azure.

Therefore, future research could explore the possibility of implementing similar architectures within these other platforms. This could involve identifying the specific services within these platforms that parallel those in AWS and adapting the architecture accordingly. Such efforts could contribute to enhancing the universality of the SPIRT architecture and its applicability across diverse cloud platforms.


\subsection{Logical Peer-to-Peer Setup}

Our research presents a unique implementation of a logical peer-to-peer (P2P) architecture within a serverless environment. Instead of conventional physical peers, our SPIRT architecture represents each peer as a logical entity consisting of an AWS Step Function instance and an associated Redis database. This abstract representation allows communication through a shared data channel rather than direct interactions, thereby combining benefits of both P2P and client-server topologies.

This approach enhances scalability and fault-tolerance, aligned with serverless computing's dynamic nature. It also mitigates potential security vulnerabilities associated with traditional P2P networks, significantly reducing the risk of peer-to-peer attacks.

\subsection{Package Management in Lambda Functions}

As highlighted in our research, the heavy dependencies of machine learning libraries pose challenges to serverless environments, primarily due to the stringent package size limits. Consequently, researchers are urged to seek innovative solutions for efficient package management. Some strategies could include eliminating unnecessary components like documentation or Cache folders, or exploring methods to compress dependencies without hampering their functionalities.


\subsection{Discussion on Failures}

In distributed environments, the aspect of failure takes on a unique dimension. Failures can occur not only on the computation units but also within the communication channels. In our architecture, communication primarily takes place through the shared database, a potential point of failure. Therefore, it's essential to consider database availability and reliability. Future work could explore strategies for database redundancy or mirroring to ensure consistent availability and mitigate potential communication channel failures.


\subsection{Implications for Reliable AI}

Reliable AI focuses on creating artificial intelligence systems that are consistent, accountable, and able to be trusted. These systems should work predictably across a range of conditions, yielding repeatable, verifiable, and explainable results. Our research on SPIRT architecture significantly aligns with and contributes to these goals.

Firstly, SPIRT operates in a serverless environment, inherently incorporating high fault-tolerance and resilience. This serverless nature mitigates potential disruptions through automated scaling, thereby ensuring reliability in AI model training. Furthermore, its design enables efficient resistance to Byzantine attacks, safeguarding the system's integrity and reinforcing the reliability of the AI outcomes under potential adversarial conditions.

Secondly, SPIRT integrates the use of RedisAI to conduct in-database model updates and gradient averaging directly within Redis. This efficient utilization of in-memory database operations minimizes network latencies and mitigates potential inconsistencies arising from network failures or fluctuations, thereby enhancing the overall reliability of the AI training process.

Lastly, the architecture leverages AWS Step Functions to construct a transparent and traceable machine learning training workflow. This clear delineation of each step in the training process promotes model interpretability, a critical aspect of Reliable AI. Every stage of the model training is explicitly tracked and auditable, facilitating transparency, accountability, and ultimately, trust in the model's results.

In essence, the SPIRT architecture fosters reliable AI by strengthening the resilience, consistency, and transparency in the AI model training process. This approach, in turn, enhances the overall trustworthiness and dependability in AI systems, a key aspect of Reliable AI.

==> 06.Discussion2.tex <==
\section{Discussions}
\label{sec:discussions}
This section critically examines the results of our study and the performance of SPIRT, identifying its implications for peer-to-peer serverless ML training and potential directions for future research.

\subsection{Security, Scalability and Fault Tolerance in Machine Learning Architecture}

In building a secure and scalable machine learning architecture, we have strived to bridge the often-opposing demands of communication efficiency, data security, and operational reliability. Our proposed architecture, with its two-tier security design and efficient communication strategies, provides a promising solution for reliable machine learning training in a decentralized environment.

The security in our architecture relies heavily on secure peer-to-peer communication and robust aggregation. We have implemented advanced cryptographic techniques to ensure data integrity, authenticity, and confidentiality, thereby significantly enhancing the security of data exchanges within the network. 

Furthering the architecture's security is the adoption of Byzantine-resilient aggregation methods. Despite the prolonged execution time compared to average aggregation, the trade-off is a necessary compromise to ensure model convergence and to protect against adversarial influences. This dual-layered security approach, bolstering secure communication and robust aggregation, serves to create a more secure and dependable environment for decentralized machine learning operations.

Beyond its security features, our architecture also demonstrates robust scalability and fault tolerance. Whether it is accommodating new peers or handling peer failures, the architecture maintains consistent performance levels and uninterrupted operations. Although the addition of new peers results in increased communication overhead, this challenge could be mitigated with advanced communication management strategies that sustain optimal performance as the network expands.

\subsection{Serverless Peer-to-Peer ML Training}

During our experimentation, we observed that batch size significantly impacts both communication overhead and training time, making it an essential factor to consider during model selection and dataset allocation.

The concept of in-database computations was another focal point in our research. By performing computations directly within the database using our bespoke RedisAI solution, we bypassed repetitive fetch-update-store cycles, effectively reducing communication overhead and enhancing system efficiency. This localized computation approach holds significant promise for future serverless distributed machine learning architectures, underlining a potential research direction exploring in-database computations' extent.

However, it's important to note that while our architecture optimizes communication overhead and training performance, the balance may shift with the addition of new peers or changes in computational workload. Therefore, continual monitoring and adaptive strategies will be needed to maintain optimal system performance.

In sum, our research offers valuable insights into the construction of secure, reliable, and efficient machine learning architectures for decentralized networks. As more machine learning processes transition towards decentralized structures, the principles and strategies elucidated in our study will be instrumental in guiding their design and functionality. Ultimately, our work contributes towards setting new standards for security, reliability, and efficiency in decentralized machine learning systems.

==> 07.ThreatsToValidity.tex <==
\section{Threats To Validity}
\label{sec:threats}


Our study on the novel Serverless Peer Integrated for Robust Training (SPIRT) architecture is not without potential threats to validity, including concerns related to internal, external, construct, and conclusion validity. However, we implemented stringent measures and experimental controls to mitigate these threats. Below, we discuss these potential risks and how we addressed each:

\subsection{Internal Validity}

\subsubsection{Hyperparameters and SPIRT Architecture}
While we strived to optimize our hyperparameters and SPIRT architecture design, it's essential to note the inherent influence these components can have on the experimental outcomes. To reduce the risk, we ran multiple iterations with different hyperparameters, ensuring our results were consistent and robust against potential biases introduced by the architecture or hyperparameters.

\subsubsection{AWS Lambda's Execution Environment}
AWS Lambda's execution environment may vary due to aspects outside of our control, potentially affecting our results. To mitigate this, we performed all our experiments within the same AWS region and during a consistent timeframe. By doing so, we aimed to reduce possible environmental variation and ensure a stable evaluation environment.

\subsection{External Validity}

\subsubsection{Model and Dataset Applicability}
While we used popular datasets (MNIST and CIFAR) and CNN models (SqueezeNet 1.1, MobileNet V3 Small, and VGG-11), the results may not directly apply to other contexts, including different datasets or more complex models. We carefully selected these datasets and models due to their wide usage and relevance in machine learning research, thus increasing the likelihood of our results being applicable to other similar contexts.

\subsection{Construct Validity}

\subsubsection{Measurement Constructs}
In our experiments, we utilized standard efficiency and performance measures. Despite these metrics being commonly used, they may not capture all performance aspects. To counteract this limitation, we employed a diverse set of metrics to provide a multifaceted view of system performance, thus improving the comprehensiveness of our evaluation.

\subsection{Conclusion Validity}

\subsubsection{Training Time Variance}
Training time is subject to variability from external factors like network conditions and availability of computational resources. However, our experimental design included repeated trials and varying conditions to ensure robust results. We also conducted our experiments within the same AWS region and timeframe to minimize environmental variability.

In conclusion, while there exist potential threats to the validity of our study, we have taken considerable measures to minimize their impact. The findings reported should be viewed within the context of these considerations. Future research can build upon this study, further refining the experimental design to validate and extend our findings.






==> Setup.tex <==
\section{Study Design}
\label{sec:study}


\begin{itemize}
    \item we optimised in both architectures by computing the average inside the database, both frameworks lambdaML, crucial and MLLESS used a database communication channel to save the intermediate gradients, then they were using other instances to pull all the gradients and make the aggregation, it was done only by leader in LambdaML. This will be costly especially when we have large gradients model.
    \item Redis vs. Postgres: This comparison is focused on saving large gradients, approximately 7Mb each, and calculating their averages. For Redis, a Lua script is utilized for the calculation of averages, while for Postgres, each gradient is stored in a table with the use of a PL script to calculate averages. For data sending operations, Redis achieves up to a 99.83\% reduction in time. In the calculation of averages, Redis achieves up to a 91.85\% decrease in time.


    \item Redis vs. Postgres: In this comparison between Redis, an in-memory key-value data store, and Postgres, a relational database, the focus is on handling large gradients, approximately 7Mb each, and computing their averages. For Redis, a Lua script is used to calculate averages, while in Postgres, each gradient is stored in a table with a PL script employed to perform the averaging. 
    When comparing the performance of data sending operations, Redis considerably outperforms Postgres by achieving up to a 99.83\% reduction in time. Similarly, in the computation of averages, Redis demonstrates its efficiency by delivering up to a 91.85\% decrease in time. These findings underline the superior performance of Redis in these tasks, leveraging its in-memory capabilities to optimally handle large-scale data.

    \item average of failure rate increase when the job size increase as well reaching 26\% of failure rate with large jobs \cite{li2014scaling}.

    \item comparing the batching and both architectures with figure

\end{itemize}


